Convolutional neural networks compression with low rank and sparse tensor decompositions

Convolutional neural networks show outstanding results in a variety of computer vision tasks. However, a neural network architecture design usually faces a trade-off between model performance and computational/memory complexity. For some real-world applications, it is crucial to develop models, which can be fast and light enough to run on edge systems and mobile devices. However, many modern architectures that demonstrate good performance don't satisfy inference time and storage limitation requirements. Thus, arises a problem of neural network compression to obtain a smaller and faster model, which is on par with the initial one. In this work, we consider a neural network compression method based on tensor decompositions. Namely, we propose to approximate the convolutional layer weight with a tensor, which can be represented as a sum of low-rank and sparse components. The motivation for such approximation is based on the assumption that low-rank and sparse terms allow eliminating two different types of redundancy and thus yield a better compression rate. An efficient CPU implementation for the proposed method has been developed. Our algorithm has demonstrated up to 3.5x CPU layer speedup and 11x layer size reduction when compressing Resnet50 architecture for the image classification task.

==> chapters/abstract.tex <==
Convolutional neural networks show outstanding results in a variety of computer vision tasks. However, a neural network architecture design usually faces a trade-off between model performance and computational/memory complexity. For some real-world applications, it is crucial to develop models, which can be fast and light enough to run on edge systems and mobile devices.  However, many modern architectures that demonstrate good performance don't satisfy inference time and storage limitation requirements.  Thus, arises a problem of neural network compression to obtain a smaller and faster model, which is on par with the initial one. 

In this work, we consider a neural network compression method based on tensor decompositions. Namely, we propose to approximate the convolutional layer weight with a tensor, which can be represented as a sum of low-rank and sparse components. The motivation for such approximation is based on the assumption that low-rank and sparse terms allow eliminating two different types of redundancy and thus yield a better compression rate. An efficient CPU implementation for the proposed method has been developed.  Our algorithm has demonstrated up to 3.5x CPU layer speedup and 11x layer size reduction when compressing Resnet50 architecture for the image classification task.

==> chapters/abstract_rus.tex <==
Сверточные нейронные сети демонстрируют поразительные результаты в самых \\разнообразных задачах машинного зрения, но при их проектировании часто необходимо искать компромисс между сложностью модели (и, соответственно, ее репрезентативностью) и ее размером (включающим в себя количество параметров и скоростью работы). Для некоторых задач реального мира полезно иметь модель, работающую с приемлемым качеством в реальном времени на устройствах с малым количеством вычислительных ресурсов, тем не менее, многие из современных моделей машинного зрения не удовлетворяют возникающим ограничениям. В таких случаях ставится задача о сжатии нейросетей - выборе наименее избыточного \\представления ее весов с минимально возможными потерями в качестве.
\par
В рамках данной работы рассматривается один из способов сжатия сверточных нейронных сетей - разложение тензора весов каждого отдельного сверточного слоя в сумму низкоранговой и разреженной части. Исследуемая гипотеза заключается в том, что низкоганговая и разреженная часть позволяют избавиться от избыточности разных типов и, таким образом, в комбинации позволяют получить более высокий уровень сжатия. Разработанная процедура разложения весов нейросети позволяет добиться до 11х сжатия сверточного слоя с ускорением до 3.5 раз на CPU без глубокой оптимизации алгоритма свертки под специфику используемого разложения. 


==> chapters/cover.tex <==
% Everything with --rus inside is supposed to be written in russian

\title{Convolutional neural networks compression with low rank and sparse tensor decompositions}
\titlerus{Сжатие сверточных нейронных сетей с применением низкоранговых и разреженных тензорных разложений}

\author{Kaloshin Pavel}
\authorrus{Калошин Павел}

\department{Data Science}
\departmentrus{Наука о данных}

\degree{Master}
\degreerus{Магистр}

\degreemonth{June}
\degreeyear{2020}
\thesisdate{June 18, 2020}
\degreemonthrus{Июнь}
\thesisdaterus{Июнь 18, 2020}

%\supervisor{Anh-Huy Phan}{Associate Professor}{Center for Computational and Data-Intensive Science and Engineering}
%\supervisorrus{Ан-Хуэй Фан}{Доцент}{Центр по научным и инженерным вычислительным технологиям для задач с большими массивами данных}

\supervisor{Anh-Huy Phan}{Associate Professor of Skoltech, Center for Computational and Data-Intensive Science and Engineering}{Ph.D}
\supervisorrus{Ан-Хуэй Фан}{Доцент Схолтеха, Центр по научным и инженерным вычислительным технологиям для задач с большими массивами данных}{Доктор наук}


\maketitle
%\rusmaketitle

\setcounter{savepage}{\thepage}
\begin{abstractpage}
\input{chapters/abstract}
\end{abstractpage}

 %\setcounter{page}{\thesavepage}
 %\begin{abstractpagerus}
 %\input{chapters/abstract_rus}
 %\end{abstractpagerus}


\section*{\centering Acknowledgments}

This work, as it is often the case, wasn't possible without the participation of different people, and I want to show my gratitude now. I want to thank my research advisor, Anh Huy Phan, for providing the idea that was a key to everything and wise guidance through the overall process, and my colleagues, Julia Gusak and Philip Blagoveschensky, for useful insights about technical implementations and inspiring discussions about the further applications.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -*-latex-*-

